Deep Learning for Human Locomotion Analysis in Lower-Limb Exoskeletons: A Comparative Study

Wearable robotics for lower-limb assistance have become a pivotal area of research, aiming to enhance mobility for individuals with physical impairments or augment the performance of able-bodied users. Accurate and adaptive control systems are essential to ensure seamless interaction between the wearer and the robotic device, particularly when navigating diverse and dynamic terrains. Despite the recent advances in neural networks for time series analysis, no attempts have been directed towards the classification of ground conditions, categorized into five classes and subsequently determining the ramp's slope and stair's height. In this respect, this paper presents an experimental comparison between eight deep neural network backbones to predict high-level locomotion parameters across diverse terrains. All the models are trained on the publicly available CAMARGO 2021 dataset. IMU-only data equally or outperformed IMU+EMG inputs, promoting a cost-effective and efficient design. Indeeds, using three IMU sensors, the LSTM achieved high terrain classification accuracy (0.94 +- 0.04) and precise ramp slope (1.95 +- 0.58{\deg}) and the CNN-LSTM a stair height (15.65 +- 7.40 mm) estimations. As a further contribution, SHAP analysis justified sensor reduction without performance loss, ensuring a lightweight setup. The system operates with ~2 ms inference time, supporting real-time applications. The code is code available at https://github.com/cosbidev/Human-Locomotion-Identification.

==> CoseVecchie.tex <==
\section{Introduction}

The field of lower limb robotics for rehabilitation and assistance employs advanced robotic technologies to support individuals with lower limb impairments or disabilities~\cite{diaz2011lower}. 
The integration of robotics into clinical practice, such as wearable exoskeletons that enhance natural movement~\cite{lee2020lower}, robotic prosthesis
\textcolor{blue}{that allow the users with artificial limbs to rewalk}~\cite{o2019prosthetic}, and rehabilitation robots designed for targeted exercises, offer significant potential for improving outcomes  \textcolor{blue}{of patients suffering from various conditions ranging from neurological up to musculoskeletal ones \cite{valgeirsdottir2022we}}.
These technologies offer several benefits, including enhanced rehabilitation, increased independence, and personalized solutions. 
However, it is crucial to provide adequate data-extracted parameters to ensure the proper functioning of lower limb exoskeletons and generate contest-adapted interventions.  
Specifically, lower-limb robots should be capable of considering different gait parameters in the control strategies according to the specific terrain conditions~\cite{gao2023autonomous}. 
While various state-of-the-art technologies allow us to perform these tasks, challenges remain, particularly in the need to equip the patient with multiple sensors and the difficulties in processing the collected data~\cite{martinez2017simultaneous, yang2019review}.
Furthermore, quickly understanding terrain characteristics and slopes with a minimal sensor set is essential to avoid obtrusive interfaces and alleviate the user's cognitive burden. Recognizing the terrain and its slope allows the robot to adjust its movements and maintain stability, improving user experience and enhancing safety.

This paper comprehensively reviews state-of-the-art supervised approaches utilized in lower limb robotics, alongside a comparative analysis of the most advanced neural network (NN)-based classifiers to identify ground conditions, categorized into five classes, i.e. level ground, stair ascent, stair descent, ramp ascent, and ramp descent, and subsequently determining the ramp's slope and stair's height using multimodal signals collected from the CAMARGO dataset.
%%Metto le due domande
{\color{blue}The objective of the paper is to propose a neural-network based systems}
Those objectives can be summarized in the answering of the next three point: 
\begin{enumerate} 
	\item We present a robust comparative analysis of models used for time series classification and regression within the domain of multimodal human locomotion \textcolor{red}{with a leave-one-subject-out cross-validation approach}
	\item \textcolor{red}{We compare multimodal and unimodal setups to evaluate whether a multimodal configuration offers any advantage over a unimodal approach. Using Explainable AI, we identify the most influential features—here, corresponding to unimodal sensor signals—and then perform an ablation study to determine the minimal sensor configuration that achieves optimal performance.} 
\end{enumerate}

The rest of the manuscript is structured as follows: \autoref{sc:sota} comprehensively reviews pertinent literature. 
\autoref{sc:materials} describes the dataset, detailing the pre-processing methodologies adopted. 
\autoref{sc:methods} describes the proposed approach and the experimental setup details, while~\autoref{sc:results} shows and discusses the results. 
Lastly,~\autoref{sc:concl} presents concluding remarks and potential future research avenues.

\subsection{Releted work}
\label{sc:sota}
Human locomotion analysis plays a crucial role in lower limb robotics, particularly in developing assistive devices such as prosthetics and exoskeletons. Wearable sensors have become essential for capturing locomotion data and providing detailed insights into human movement. Two widely used sensors in this field are Inertial Measurement Units (IMUs) and electromyography (EMG) sensors~\cite{ribeiro2017inertial}.
Purhereas the latter sensors, conversely, detect muscle activity, offering insights into neuromuscular function movement patterns during various locomotion tasks~\cite{gupta2017semg, sorkhabadi2019human, bartlett2017phase}.

Traditional machine learning algorithms such as k-Nearest Neighbor (k-NN), Support Vector Machines (SVM), Gaussian Mixture Models (GMM), and Random Forests (RF) have been widely applied to time series classification to classify locomotion data derived from IMU and EMG sensors. 
However, these methods rely on manual feature extraction, which requires significant expertise and effort. 
This limitation has led to increasing interest in deep learning (DL) techniques that automate feature extraction through neural networks (NNs)~\cite{attal2015physical}.

Although presenting a detailed review of these methods in the literature is out of the scope of this manuscript, the information reported in Table \ref{tab:soa} suggests that most of the works performed focus on an unimodal approach and just three have performed and multimodal analysis \cite{negi2020human, zhang2020unsupervised, zhao2022multi}. 
\textcolor{red}{It is known that  the multimodal approach
is useful to solve complex tasks, and early fusion is used in such three works. In early
 fusion, raw input data is combined into a shared embedded space using various strategies, such as simple
 concatenation, addition, pooling, or by applying a gated unit.}
While this approach has shown promising results across several applications, and complex tasks, there are still key challenges to address. These include managing one or more missing modalities, handling different sampling rates and/or time synchronization between multiple data sources, and dealing with potential redundancies that arise when generating large embedded spaces \cite{tortora2023radiopathomics}.
%Limiti della letteratura
The current limitations of the literature include the lack of a neural network-based system capable of classifying locomotion and predicting ramp inclination or step height. To address this limitation, we conducted a comparative study of eight different methods to identify the best one. Another limitation is the absence of a multimodal study to determine the optimal modality. Furthermore, for real-life applications, it is also crucial to perform an accurate analysis of the minimum number of sensors that can be mounted on a robot. To address this limitation, we employed an explainable AI method called SHAP.
\begin{landscape}
\input{table_stato_dell_arte}
\end{landscape}


\begin{table}[h!]
\centering
\caption{ \textcolor{red}{Classification Results: Displaying the Mean Performance and Variability Across Metrics}}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc|}
\cline{2-7}
                               & \multicolumn{3}{c|}{Classification Accuracy}  & \multicolumn{3}{c|}{Training Time x 1 epoch [s]} \\ \hline
\multicolumn{1}{|c|}{\textbf{Architecture}} &
  \textbf{IMU} &
  \textbf{EMG} &
  \textbf{IMU + EMG} &
  \textbf{IMU} &
  \textbf{EMG} &
  \textbf{IMU + EMG} \\ \hline
\multicolumn{1}{|c|}{CNN}      & $0.92\pm0.05$ & $0.73\pm0.1$  & $0.92\pm0.04$ & $13.23 \pm 0.24$   & $15.45 \pm 0.35$   & $16.34 \pm 0.42$   \\
\multicolumn{1}{|c|}{LSTM} &
  $\mathbf{0.94\pm0.04}$ &
  $0.60\pm0.06$ &
  $\mathbf{0.94\pm0.03}$ &
  $21.14 \pm 0.35$ &
  $24.54 \pm 0.65$ &
  $26.35 \pm 0.27$ \\
\multicolumn{1}{|c|}{CNN-LSTM} & $0.90\pm0.05$ & $0.75\pm0.08$ & $0.93\pm0.04$ & $11.42 \pm 0.15$   & $12.34 \pm 0.37$   & $14.53 \pm 0.24$   \\
\multicolumn{1}{|c|}{LSTM-CNN} & $0.91\pm0.05$ & $0.75\pm0.1$  & $0.91\pm0.04$ & $16.23 \pm 0.54$   & $17.43 \pm 0.34$   & $17.43 \pm 0.24$   \\
\multicolumn{1}{|c|}{GRU}      & $0.78\pm0.08$ & $0.61\pm0.03$ & $0.79\pm0.07$ & $21.67 \pm 0.41$   & $23.45 \pm 0.56$   & $25.45 \pm 0.14$   \\
\multicolumn{1}{|c|}{TST}      & $0.92\pm0.04$ & $0.74\pm0.03$ & $0.91\pm0.05$ & $17 \pm 0.31$      & $18.33 \pm 0.14$   & $18.23 \pm 0.45$   \\
\multicolumn{1}{|c|}{XceptionTime} &$0.88\pm0.09$ &$0.73\pm0.03$ &$0.89\pm0.09$ &$55.19 \pm 0.57$ &$66.09 \pm 0.35$ &$66.62 \pm 0.48$ \\
\multicolumn{1}{|c|}{Mamba} & $0.92\pm0.04$ &$\mathbf{0.76\pm0.05}$ &$0.91\pm0.06$ &$14.256\pm 0.25$ &$15.56 \pm 0.25$ &$15.93 \pm 0.37$ \\
\multicolumn{1}{|c|}{Mean} & $0.89\pm0.05$ &$0.71\pm0.06$ &$0.90\pm0.05$ &$21.25\pm 0.35$ &$24.14 \pm 0.37$ &$25.11 \pm 0.32$ \\ \hline
\end{tabular}%
}
\end{table}

\begin{table}[h!]
\centering
\caption{Supplementary Metrics with Standard Deviation}
\label{tab:my-table5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc|}
\cline{2-10}
 & \multicolumn{3}{c|}{\textbf{Precision}} & \multicolumn{3}{c|}{\textbf{Recal}} & \multicolumn{3}{c|}{\textbf{F1 Score}} \\ 
\hline
\multicolumn{1}{|c|}{\textbf{Architecture}} & 
  \textbf{IMU} & 
  \textbf{EMG} & 
  \textbf{IMU + EMG} & 
  \textbf{IMU} & 
  \textbf{EMG} & 
  \textbf{IMU + EMG} & 
  \textbf{IMU} & 
  \textbf{EMG} & 
  \textbf{IMU + EMG} \\ 
\hline
\multicolumn{1}{|c|}{CNN}      & $0.92\pm0.03$& $0.79\pm0.15$   & $0.92\pm0.06$  &$0.89\pm0.08$ & $0.73\pm0.04$ & $0.91\pm0.06$ & $0.89\pm0.05$ & $0.74\pm0.07$ & $0.91\pm0.06$ \\
\multicolumn{1}{|c|}{LSTM}     & ${0.95\pm0.04}$ & ${0.39\pm0.07}$ & $0.95\pm0.05$  & $0.94\pm0.06$ & ${0.60\pm0.07}$ & $0.94\pm0.08$ &$0.94\pm0.05$  & ${0.46\pm0.07}$ & $0.94\pm0.06$ \\
\multicolumn{1}{|c|}{CNN-LSTM} & $0.93\pm0.05$ & ${0.80\pm0.04}$  & $0.93\pm0.07$   & $0.92\pm0.05$ & ${0.75\pm0.03}$ & $0.90\pm0.07$  & $0.92\pm0.08$& ${0.76\pm0.03}$ & $0.91\pm0.07$  \\
\multicolumn{1}{|c|}{LSTM-CNN} & $0.93\pm0.07$ & $0.78\pm0.04$   & $0.92\pm0.08$   & $0.91\pm0.03$ & $0.75\pm0.09$ & $0.90\pm0.06$  &$0.91\pm0.04$ & $0.76\pm0.06$ & $0.90\pm0.05$  \\
\multicolumn{1}{|c|}{GRU}      & $0.78\pm0.07$ & $0.61\pm0.02$ & $0.78\pm0.06$ & $0.77\pm0.08$ & $0.60\pm0.03$ & $0.77\pm0.06$ & $0.79\pm0.07$ & $0.60\pm0.03$ & $0.79\pm0.1$ \\
\multicolumn{1}{|c|}{TST}      & $0.92\pm0.04$ & $0.75\pm0.03$  & $0.91\pm0.04$  & $0.92\pm0.04$ & $0.74\pm0.02$ & $0.91\pm0.04$ & $0.92\pm0.05$ & $0.74\pm0.03$& $0.91\pm0.05$ \\
\multicolumn{1}{|c|}{XceptionTime} & $0.88\pm0.09$ & $0.73\pm0.03$  & $0.88\pm0.01$  & $0.90\pm0.05$ & $0.74\pm0.03$ & $0.89\pm0.05$ & $0.88\pm0.09$ & $0.73\pm0.03$ & $0.88\pm0.09$ \\
\multicolumn{1}{|c|}{Mamba}    & $0.92\pm0.05$& $0.75\pm0.05$  & $0.91\pm0.05$  & $0.89\pm0.05$ & $0.73\pm0.05$ & $0.91\pm0.05$ & $0.89\pm0.05$ & $0.75\pm0.05$ & $0.92\pm0.05$ \\
\multicolumn{1}{|c|}{Mean}     & $0.90\pm0.05$ & $0.70\pm0.05$  & $0.90\pm0.05$  & $0.89\pm0.06$ & $0.71\pm0.06$ & $0.89\pm0.07$ & $0.89\pm0.06$ & $0.78\pm0.05$ & $0.89\pm0.07$ \\ 
\hline
\end{tabular}%
}
\end{table}

\begin{table}[]
\centering
\caption{\textcolor{red}{Regression Analysis of Slope Inclination and Stair Height: Predictive Performance and Trends}}
\label{tab:my-table2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc|}
\cline{2-5}
                                   & \multicolumn{2}{c|}{Slope}                & \multicolumn{2}{c|}{Height}                \\ \hline
\multicolumn{1}{|c|}{Architecture} & MAE [$\mathbf{^\circ}$] & Training time [s] & MAE [mm] & Training time [s] \\ \hline
\multicolumn{1}{|c|}{CNN}          & $2.21\pm0.58$          & $13.57 \pm 0.17$ & $18.00\pm8.51$          & $10.09 \pm 0.36$ \\
\multicolumn{1}{|c|}{LSTM}         & $\mathbf{1.93\pm0.53}$ & $25 \pm 0.37$    & $15.97\pm6.29$          & $20.35 \pm 0.48$ \\
\multicolumn{1}{|c|}{CNN-LSTM}     & $2.10\pm0.68$          & $14.76 \pm 0.38$ & $\mathbf{15.65\pm6.33}$ & $11 \pm 0.45$    \\
\multicolumn{1}{|c|}{LSTM-CNN}     & $2.14\pm0.73$          & $20 \pm 0.37$    & $16.05\pm7.40$          & $16 \pm 0.77$    \\
\multicolumn{1}{|c|}{GRU}          & $2.32\pm0.61$          & $23.45 \pm 0.65$ & $21.10\pm9.11$          & $19.59 \pm 0.78$ \\
\multicolumn{1}{|c|}{TST}          & $2.21\pm0.60$          & $16.34 \pm 0.26$ & $17.56\pm6.65$          & $13.45 \pm 0.56$ \\
\multicolumn{1}{|c|}{XceptionTime} & $2.08\pm0.54$          & $64.34 \pm 0.23$ & $17.30\pm7.57$          & $58.45 \pm 0.36$ \\
\multicolumn{1}{|c|}{Mamba}        & $2.03\pm0.46$          & $14.56 \pm 0.24$ & $16.02\pm6.89$          & $12.45 \pm 0.13$ \\
\multicolumn{1}{|c|}{Mean}         & $2.12\pm0.59$          & $24.00\pm0.33$   & $17.20\pm7.34$          & $20.14\pm0.46$   \\ \hline
\end{tabular}%
}
\end{table}

$Intro$

{\color{red}The field of lower limb robotics for rehabilitation and assistance employs advanced robotic technologies to support individuals with lower limb impairments or disabilities~\cite{diaz2011lower}. In particular, the integration of robotics into clinical practice—ranging from wearable exoskeletons that enhance natural movement~\cite{lee2020lower} to robotic prostheses that allow users with artificial limbs to walk again~\cite{o2019prosthetic}, and rehabilitation robots designed for targeted exercises~\cite{valgeirsdottir2022we}—offers significant potential for improving patient outcomes. These technologies provide enhanced rehabilitation, increased independence, and personalized solutions. However, ensuring their effective operation requires adequate data-extracted parameters and context-adapted interventions. Specifically, lower-limb robots need to consider different gait parameters in their control strategies according to specific terrain conditions~\cite{gao2023autonomous}.

While various state-of-the-art technologies enable this, several challenges persist. Notably, many approaches require equipping the patient with multiple sensors and involve the complex processing of the collected data~\cite{martinez2017simultaneous, yang2019review}. A key requirement for a more user-friendly system is the rapid and accurate understanding of terrain characteristics and slopes with a minimal sensor setup, which helps avoid obtrusive interfaces and reduces the user’s cognitive burden. Recognizing the terrain type and its slope enables the robot to adapt its movements and maintain stability, thereby improving the user experience and enhancing safety.

Human locomotion analysis is critical in lower limb robotics, particularly in developing assistive devices such as prosthetics and exoskeletons. Wearable sensors have become integral to capturing locomotion data and providing detailed insights into human movement. Two widely used sensor types in this context are Inertial Measurement Units (IMUs), which measure acceleration and angular velocity to capture body orientation and movement~\cite{ribeiro2017inertial}, and electromyography (EMG) sensors, which detect muscle activity to reveal neuromuscular function and movement patterns~\cite{gupta2017semg, sorkhabadi2019human, bartlett2017phase}.

Traditional machine learning algorithms—such as k-Nearest Neighbor (k-NN), Support Vector Machines (SVM), Gaussian Mixture Models (GMM), and Random Forests (RF)—have been widely employed for time series classification of locomotion data collected via IMU and EMG sensors. However, these methods rely on manual feature extraction, a time-consuming process requiring substantial expertise~\cite{attal2015physical}. Consequently, there has been increasing interest in deep learning (DL) approaches for automating feature extraction and classification tasks through neural networks (NNs).

Despite notable progress in unimodal setups, a growing body of work demonstrates the benefits of multimodal sensor fusion. As summarized in Table~\ref{tab:soa}, most approaches remain unimodal, with only three studies performing multimodal analyses~\cite{negi2020human, zhang2020unsupervised, zhao2022multi}. These multimodal methods generally apply an early-fusion strategy—merging raw data into a shared embedded space through concatenation, addition, pooling, or the use of gated units~\cite{tortora2023radiopathomics}. While multimodal sensor fusion can offer improved performance in complex tasks, unresolved challenges include accommodating missing or misaligned modalities with different sampling rates and minimizing redundancies that create excessively large embedded spaces.

Additionally, existing literature on neural-network-based systems for lower limb robotics typically focuses on classification tasks alone (e.g., locomotion mode detection) and often does not extend to predictions such as ramp inclination or step height. Moreover, few studies comprehensively investigate the minimum number of sensors required for robust performance—an aspect critical for real-life applications where reducing complexity and cost is paramount.

In this paper, we address these gaps by proposing a neural-network-based system that classifies ground conditions (level ground, stair ascent, stair descent, ramp ascent, and ramp descent) and also predicts ramp inclination or step height using multimodal signals from the CAMARGO dataset. Specifically: 
\begin{enumerate} 
\item We present a robust comparative analysis of eight models commonly used for time series classification and regression within the domain of multimodal human locomotion. A leave-one-subject-out cross-validation approach is employed to ensure generalizability. \item We compare multimodal and unimodal setups to determine whether a multimodal configuration offers any advantage over a unimodal approach. Using Explainable AI techniques, we identify the most influential features—here, corresponding to unimodal sensor signals—and then conduct an ablation study to establish the minimal sensor configuration that achieves optimal performance. \end{enumerate}
The rest of the manuscript is organized as follows. Section~\ref{sc:materials} describes the dataset and the adopted pre-processing methods. Section~\ref{sc:methods} elaborates on the proposed neural network approaches and the experimental setup. Section~\ref{sc:results} presents and discusses the results, while Section~\ref{sc:concl} provides concluding remarks and outlines potential future research directions.}


\begin{comment}
\begin{table}[h!]
\centering
\caption{Comparison of architectures for classification task based on accuracy.
Bold font is used to highlight the best results for each modality.}
\label{tab:times}
\begin{tabular}{cccc} 
\toprule
\textbf{Architecture}  & \textbf{IMU} & \textbf{EMG} & \textbf{IMU + EMG}\\  
\midrule
CNN & $0.92\pm0.05$ & $0.73\pm0.1$ & $0.92\pm0.04$ \\  
LSTM & $\mathbf{0.94\pm0.04}$ & $0.60\pm0.06$ & $\mathbf{0.94\pm0.03}$ \\   
CNN-LSTM & $0.90\pm0.05$ & $0.75\pm0.08$ & $0.93\pm0.04$  \\ 
LSTM-CNN & $0.91\pm0.05$ & $0.75\pm0.1$ & $0.91\pm0.04$ \\
GRU & $0.78\pm0.08$ &$0.61\pm0.03$& $0.79\pm0.07$  \\
TST & $0.92\pm0.04$ &$0.74\pm0.03$& $0.91\pm0.05$ \\
XceptionTime & $0.88\pm0.09$ & $0.73\pm0.03$& $0.89\pm0.09$\\
Mamba & $0.92\pm0.04$ & $\mathbf{0.76\pm0.05}$ & $0.91\pm0.06$ \\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\hline
         & \multicolumn{3}{c}{Classification Accuracy}   & \multicolumn{3}{c}{Training Time x 1 epoch [s]} \\ \hline
\textbf{Architecture} & \textbf{IMU}           & \textbf{EMG}           & \textbf{IMU + EMG}     & \textbf{IMU}     & \textbf{EMG}     & \textbf{IMU + EMG} \\ \hline
CNN      & $0.92\pm0.05$ & $0.73\pm0.1$  & $0.92\pm0.04$ & $13.23 \pm 0.24$   & $15.45 \pm 0.35$   & $16.34 \pm 0.42$  \\
LSTM                  & $\mathbf{0.94\pm0.04}$ & $0.60\pm0.06$          & $\mathbf{0.94\pm0.03}$ & $21.14 \pm 0.35$ & $24.54 \pm 0.65$ & $26.35 \pm 0.27$   \\
CNN-LSTM & $0.90\pm0.05$ & $0.75\pm0.08$ & $0.93\pm0.04$ & $11.42 \pm 0.15$   & $12.34 \pm 0.37$   & $14.53 \pm 0.24$  \\
LSTM-CNN & $0.91\pm0.05$ & $0.75\pm0.1$  & $0.91\pm0.04$ & $16.23 \pm 0.54$   & $17.43 \pm 0.34$   & $17.43 \pm 0.24$  \\
GRU      & $0.78\pm0.08$ & $0.61\pm0.03$ & $0.79\pm0.07$ & $21.67 \pm 0.41$   & $23.45 \pm 0.56$   & $25.45 \pm 0.14$  \\
TST      & $0.92\pm0.04$ & $0.74\pm0.03$ & $0.91\pm0.05$ & $17.00 \pm 0.31$      & $18.33 \pm 0.14$   & $18.23 \pm 0.45$  \\
XceptionTime          & $0.88\pm0.09$          & $0.73\pm0.03$          & $0.89\pm0.09$          & $55.19 \pm 0.57$ & $66.09 \pm 0.35$ & $66.62 \pm 0.48$   \\
Mamba                 & $0.92\pm0.04$          & $\mathbf{0.76\pm0.05}$ & $0.91\pm0.06$          & $14.256\pm 0.25$ & $15.56 \pm 0.25$ & $15.93 \pm 0.37$   \\ \hline
\end{tabular}%
}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[h!]
\centering
\caption{\textcolor{red}{Regression Analysis of Slope Inclination and Stair Height: Predictive Performance and Trends}}
\label{tab:my-table2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Architecture}} & \textbf{MAE [$\mathbf{^\circ}$] (Slope)} & \textbf{MAE [mm] (Height)} \\ \hline
\multicolumn{1}{|c|}{CNN}          & $2.21\pm0.58$          & $18.00\pm8.51$  \\
\multicolumn{1}{|c|}{LSTM}         & $\mathbf{1.93\pm0.53}$ & $15.97\pm6.29$  \\
\multicolumn{1}{|c|}{CNN-LSTM}     & $2.10\pm0.68$          & $\mathbf{15.65\pm6.33}$  \\
\multicolumn{1}{|c|}{LSTM-CNN}     & $2.14\pm0.73$          & $16.05\pm7.40$  \\
\multicolumn{1}{|c|}{GRU}          & $2.32\pm0.61$          & $21.10\pm9.11$  \\
\multicolumn{1}{|c|}{TST}          & $2.21\pm0.60$          & $17.56\pm6.65$  \\
\multicolumn{1}{|c|}{XceptionTime} & $2.08\pm0.54$          & $17.30\pm7.57$  \\
\multicolumn{1}{|c|}{Mamba}        & $2.03\pm0.46$          & $16.02\pm6.89$  \\
\multicolumn{1}{|c|}{Mean}         & $2.12\pm0.59$          & $17.20\pm7.34$  \\ \hline
\end{tabular}%
}
\end{table}
\end{comment}


\begin{comment}
    
\begin{table}[]
\centering
\caption{\textcolor{red}{Regression Analysis of Slope Inclination and Stair Height: Predictive Performance and Trends}}
\label{tab:my-table2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc|}
\cline{2-5}
                                   & \multicolumn{2}{c|}{Slope}                & \multicolumn{2}{c|}{Height}                \\ \hline
\multicolumn{1}{|c|}{Architecture} & MAE [$\mathbf{^\circ}$] & Training time [s] & MAE [mm] & Training time [s] \\ \hline
\multicolumn{1}{|c|}{CNN}          & $2.21\pm0.58$          & $13.57 \pm 0.17$ & $18.00\pm8.51$          & $10.09 \pm 0.36$ \\
\multicolumn{1}{|c|}{LSTM}         & $\mathbf{1.93\pm0.53}$ & $25 \pm 0.37$    & $15.97\pm6.29$          & $20.35 \pm 0.48$ \\
\multicolumn{1}{|c|}{CNN-LSTM}     & $2.10\pm0.68$          & $14.76 \pm 0.38$ & $\mathbf{15.65\pm6.33}$ & $11 \pm 0.45$    \\
\multicolumn{1}{|c|}{LSTM-CNN}     & $2.14\pm0.73$          & $20 \pm 0.37$    & $16.05\pm7.40$          & $16 \pm 0.77$    \\
\multicolumn{1}{|c|}{GRU}          & $2.32\pm0.61$          & $23.45 \pm 0.65$ & $21.10\pm9.11$          & $19.59 \pm 0.78$ \\
\multicolumn{1}{|c|}{TST}          & $2.21\pm0.60$          & $16.34 \pm 0.26$ & $17.56\pm6.65$          & $13.45 \pm 0.56$ \\
\multicolumn{1}{|c|}{XceptionTime} & $2.08\pm0.54$          & $64.34 \pm 0.23$ & $17.30\pm7.57$          & $58.45 \pm 0.36$ \\
\multicolumn{1}{|c|}{Mamba}        & $2.03\pm0.46$          & $14.56 \pm 0.24$ & $16.02\pm6.89$          & $12.45 \pm 0.13$ \\
\multicolumn{1}{|c|}{Mean}         & $2.12\pm0.59$          & $24.00\pm0.33$   & $17.20\pm7.34$          & $20.14\pm0.46$   \\ \hline
\end{tabular}%
}
\end{table}
\end{comment}

==> tabellaaggiuntiva.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Literature analysis on the existing methodologies for locomotion classification and incline prediction.}
\label{tab:soa}
\begin{tabular}{ccccc}
\toprule
Ref. & Modality & Algorithm & Accuracy [\%] & Dataset \\ \midrule
\cite{negi2020human}   &  EMG and acceleration       &  LDA, KNN, DT, RF, SVM      & 0.97, 0.98, 0.79, 0.80, 0.99    &  Collected within the paper (CWP)     \\
\cite{zhang2020unsupervised}   &    EMG and IMU      &     LDA, SVM, ANN, CNN, DANN, MCD      &    0.92, 0.90, 0.93, 0.96, 0.95, 0.95     & ENABL3S and DSADS   \\
\cite{narayan2021real}   &    IMU      &     CNN      &     0.94     &   CWP   \\
\cite{amer2021human}   &    IMU      &     CNN      &     0.99     &    CWP    \\
\cite{azmat2021smartphone}   &    IMU      &    New Proposed Algorithm     &     0.84     &   MobiAct dataset   \\
\cite{wang2022locomotion}   &    IMU      &     Residual Network      &     0.97    &   CWP     \\
\cite{zhao2022multi}   &    EMG and IMU      &    CNN      &     0.94     &   ENABL3S public dataset    \\
\cite{jing2022accurate}   &    EMG      &    CNN      &     0.97  &   HDsEMG dataset   \\
\cite{zheng2022cnn}   &    IMU      &     SVM, CNN      &     0.98, 0.99     &   CWP   \\
\cite{le2022deep}   &    IMU      &     CNN      &     0.74     &   ENABL3S    \\
\cite{kang2022subject}   &    IMU      &   CNN      &     0.93     &  CAMARGO 2021    \\
\cite{son2023multivariate}   &    IMU      &    CNN-LSTM, LSTM-CNN      &     0.94, 0.95     &   CWP    \\ \bottomrule   
\end{tabular}
\end{table*}
